To be or not to be stable, that is the question: understanding neural networks for inverse problems

The solution of linear inverse problems arising, for example, in signal and image processing is a challenging problem since the ill-conditioning amplifies, in the solution, the noise present in the data. Recently introduced algorithms based on deep learning overwhelm the more traditional model-based approaches in performance, but they typically suffer from instability with respect to data perturbation. In this paper, we theoretically analyze the trade-off between stability and accuracy of neural networks, when used to solve linear imaging inverse problems for not under-determined cases. Moreover, we propose different supervised and unsupervised solutions to increase the network stability and maintain a good accuracy, by means of regularization properties inherited from a model-based iterative scheme during the network training and pre-processing stabilizing operator in the neural networks. Extensive numerical experiments on image deblurring confirm the theoretical results and the effectiveness of the proposed deep learning-based approaches to handle noise on the data.

==> inverse_problems.tex <==
\section{Inverse Problems}

\subsection{Direct Approach to Inverse Problems}
Many physical phenomenon can be modelled as the result of the application of a linear operator $\mathcal{K}: L^2(\R^2) \to L^2(\R^2)$ to an (unknown) image $f \in L^2(\R^2)$ via the so-called First Kind Fredholm Equation:

\begin{align}\label{eq:fred_eq}
    g(s, t) = (\mathcal{K}f)(s, t) = \int_{\R^2} k(\x, y; \xi, \eta)f(\xi, \eta)d\xi d\eta
\end{align}

Here the kernel $k(s, t; \xi, \eta)$ it usually considered to be spatial invariant (i.e. $k(s, t; \xi, \eta) = k(s-\xi, t-\eta)$). When is happens, $k(s, t)$ is called \emph{point spread function} (PSF). Discretizing \eqref{eq:fred_eq} on a $\sqrt{n} \times \sqrt{n}$ grid lead to

\begin{align}\label{eq:disc_fred_eq}
    y = A\x
\end{align}

where $\x, y \in \R^{n}$, $A \in \R^{n \times n}$ is an highly ill-conditioned matrix, usually with a strong structure (i.e. sparse or Toeplitz). \\

To explain the following results, recall that the Singular Value Decomposition) of $A$ is:

\begin{align}
    A = U \Sigma V^T
\end{align}

where $U,V \in \R^{n \times n}$ are orthogonal matrices, $\Sigma \in \R^{n \times n}$ is a diagonal matrix with diagonal elements $(\sigma_1, \dots, \sigma_n)^T$, where $\sigma_1 \geq \sigma_2 \geq \dots \geq \sigma_n \geq 0$ are the singular values of $A$. A matrix $A$ is singular if $\exists r < n$ s.t. $\sigma_{r+1} = \sigma_{r+2} = \dots = \sigma_n = 0$ (in this case, $A$ is a rank $r$ matrix), and is ill-conditioned if the singular values quickly decrease to 0. We will be interested in understanding the $t$-rank of $A$, which is the number of singular values greater than a fixed real number $t > 0$.

\begin{definition}
    Let $A \in \R^{n \times n}$ be a matrix and $A = U\Sigma V^T$ its SVD decomposition. Given $t>0$, we define
    \begin{align*}
        r(t) = \min \{ r \in \mathbb{N} \> | \> \sigma_r > t \} 
    \end{align*}
    if $\sigma_r > t$ $\forall r = 1, \dots, n$, then $r(t) := n$.
\end{definition}

In ill-conditioned inverse problem, usually $r(t)$ decreases very quickly as a function of $t$, and usually $r(t) < n$ even for very small values of $t$. \\

Recall that a classical solution of $y = A\x$ is 

\begin{align*}
    \tilde{\x} = V\Sigma^{-1} U^T y = \sum_{i=1}^n \frac{u_i^Ty}{\sigma_i} v_i
\end{align*}

here, if $t>0$ is fixed, we can split

\begin{align*}
    \tilde{\x} = \sum_{i=1}^{r(t)} \frac{u_i^Ty}{\sigma_i} v_i + \sum_{i=r(t)+1}^{n} \frac{u_i^Ty}{\sigma_i} v_i \geq \sum_{i=1}^{r(t)} \frac{u_i^Ty}{\sigma_i} v_i + \frac{1}{t} \sum_{i=r(t)+1}^{n}(u_i^Ty) v_i
\end{align*}

where the last term amplifies computational errors on $y$ when $r(t)<n$ for very small values of $t$. \\

To solve this problem, we introduce a (possibly non-linear) continuous reconstruction algorithm $\Psi: \R^n \to \R^n$ such that it correctly reconstructs $\x \in \R^n$ with $A\x = y$, when applied to $y$.

\begin{definition}
    A reconstruction algorithm $\Psi: \R^n \to \R^n$ has accuracy $\eta>0$ if
    \begin{align*}
        || \Psi(A\x) - \x || < \eta \> \forall \x \in \R^n
    \end{align*}
    In this case, we will write $\Psi(A\x) \approx_\eta \x$.
\end{definition}

Given a reconstruction algorithm with accuracy $\eta>0$ (which can be easily done by neural networks, as we will see), we are interested in understanding its stability, which is its behavior when its input $A\x$ is perturbed by a small-norm corruption. In particular, we give the following definition.

\begin{definition}
    Given $\delta > 0$, a reconstruction algorithm $\Psi$ with accuracy $\eta>0$ is $\delta$-stable if for any $|| e || < \delta$, 
    \begin{align}
        || \Psi(A\x + e) - \x || < C\delta + \eta
    \end{align}
    for some $C > 0$. Here, the $\eta$ term is added because we want that when $\delta = 0$, $\Psi(A\x) \approx_\eta \x$.
\end{definition}

and our goal is to find conditions such that a given reconstruction algorithm $\Psi$ with accuracy $\eta$ is $\delta$-stable for some $\delta>0$. To answer this question, we need to introduce the concept of local Lipschitz constant. Indeed, our algorithm $\Psi$ is in general continuous but not Lipschitz continuous, thus we cannot define a global Lipschitz constant.

\begin{definition}
    Given $\epsilon>0$ and $y \in \R^n$, we define the $\epsilon$-Lipschitz constant of $\Psi$ around $y$ as:
    
    \begin{align*}
        L^\epsilon(\Psi, y) = \sup_{z: ||z-y||\leq \epsilon} \frac{||\Psi(z) - \Psi(y) ||}{||z - y||}
    \end{align*}
\end{definition}

Intuitively, the concepts  of local Lipschitz constant and $\delta$-stability are strongly related, since a function with high Lipschitz constant is usually unstable. This idea is confirmed by the following Theorem.

\begin{theorem}\label{thm:lip_implies_stab}
    If $\Psi: \R^n \to \R^n$ is a continuous reconstruction algorithm with accuracy $\eta>0$, $\epsilon$-Lipschitz constant $L^\epsilon(\Psi, y)$ for any $y \in \R^n$ and $||e||\leq \epsilon$, then
    
    \begin{align}
        || \Psi(A\x + e) - \x || < L^\epsilon(\Psi, A\x) \epsilon + \eta
    \end{align}
\end{theorem}

\begin{proof}
    By the triangle inequality follows that
    \begin{align*}
        || \Psi(A\x + e) - \x || \leq || \Psi(A\x + e) - \Psi(A\x) || + || \Psi(A\x) - \x ||
    \end{align*}
    since $||e||\leq \epsilon$, it follows from the definition of local Lipschitz constant with $y = A\x$ and $z = A\x + e$ that
    \begin{align*}
        || \Psi(A\x + e) - \Psi(A\x) || \leq L^\epsilon(\Psi, A\x) || A\x + e - A\x || = L^\epsilon(\Psi, A\x) || e || \leq L^\epsilon(\Psi, A\x) \epsilon
    \end{align*}
    while the accuracy of $\Psi$ implies that
    \begin{align*}
        || \Psi(A\x) - \x || < \eta
    \end{align*}
    Joining everything together gives
    \begin{align*}
        || \Psi(A\x + e) - \x || < L^\epsilon(\Psi, A\x) \epsilon + \eta
    \end{align*}
\end{proof} 

As a consequence, if $\exists C > 0$ such that $L^\epsilon(\Psi, A\x) < C$ for any $\x \in \R^n$, then Theorem \ref{thm:lip_implies_stab} implies that $\Psi$ is $\epsilon$-stable. Unfortunately, this is not always the case.

\begin{theorem}\label{thm:estimates_of_lip}
    If $\Psi: \R^n \to \R^n$ is a continuous reconstruction algorithm with accuracy $\eta>0$, $\epsilon$-Lipschitz constant $L^\epsilon(\Psi, y)$ for any $y \in \R^n$ with $\epsilon \geq \eta$ and there are $\x, \x' \in \R^n$ such that $y = A\x$ and $|| A(\x-\x') || < \eta$, then there is a closed ball $\mathcal{B}_y \subseteq \R^n$ around $y$ such that for any $\tilde{y} \in \mathcal{B}_y$, 
    \begin{align*}
        L^\epsilon(\Psi, \tilde{y}) \geq \frac{1}{\epsilon} \Bigl(||\x - \x'|| - 2\eta \Bigr)
    \end{align*}
\end{theorem}

\begin{proof}
    Let $y = A\x$. By the definition of $\epsilon$-Lipschitz constant we have
    \begin{align*}
        L^\epsilon(\Psi, y) &= \sup_{z: ||z - y|| \leq \epsilon} \frac{|| \Psi(z) - \Psi(y) ||}{||z - y ||} \geq \frac{|| \Psi(A\x') - \Psi(A\x) ||}{||A(\x'-\x)||} = \\ &= \frac{|| \Psi(A\x') - \x' - \Psi(A\x) + \x + \x' - \x||}{||A(\x'-\x)||} \geq \\ &\geq \frac{- || \Psi(A\x') - \x' || - || \Psi(A\x) - \x || + || \x' - \x||}{||A(\x'-\x)||} > \\ & > \frac{|| \x' - \x || - 2\eta}{\eta} \overset{(\epsilon \geq \eta)}{\geq} \frac{|| \x' - \x || - 2\eta}{\epsilon}
    \end{align*}
    which implies that
    \begin{align*}
        L^\epsilon(\Psi, y) > \frac{|| \x' - \x || - 2\eta}{\epsilon}
    \end{align*}
    Continuity of $\Psi$ implies that there is a ball $\mathcal{B}_y$ around $y$ such that this estimates holds for any $\tilde{y} \in \mathcal{B}_y$.
\end{proof}

To summarize, Theorem \ref{thm:lip_implies_stab} implies that $\Psi$ is $\epsilon$-stable if its $\epsilon$-Lipschitz constant $L^\epsilon(\Psi, y)$ is bounded as a function of $\epsilon$ and $y = A\x$. Unfortunately, Theorem \ref{thm:estimates_of_lip} implies that $L^\epsilon(\Psi, y)$ is unbounded as soon as we can find $\x, \x' \in \R^n$ such that $||A(\x - \x')|| < \eta$ but $|| \x - \x' || \gg 2\eta$, with $\eta \leq \epsilon$ being the accuracy of $\Psi$. Thus, we are trying to find conditions that implies the existence of such points. We will show that their existence is strongly related to the ill-conditioning of $A$, and in particular to how quickly the function $r(t)$ shrink. \\

Let $\x \in \R^n$ and $y = A\x$. Let $(\sigma_1, \dots, \sigma_n)^T$ be the singular values of $A$ and $(v_1, \dots, v_n)^T$ the left-singular vectors associated to $(\sigma_1, \dots, \sigma_n)^T$. For any $r = 1, \dots, n$, define $V_r := Span\{ v_{r}, v_{r+1}, \dots, v_n \}$ the subspace defined by the left singular vectors of $A$ smaller then $\sigma_r$. Consider the accuracy $\eta>0$ to be fixed.

\begin{theorem}\label{thm:ill_cond_implies_existence}
    Let $t>0$ be such that $r(t)<n$ and $\eta > 0$. Then there are points $\x, \x' \in \R^n$ such that $||\x - \x' ||=\frac{\eta}{t}$ but $||A(\x-\x')||<\eta$. In particular, for every $\x \in \R^n$, there are $\infty^{n - r(t)}$ $\x' \in \R^n$ such that the estimate above holds.
\end{theorem}  

\begin{proof}
    Let $t>0$ be fixed such that $r(t)<n$. Consider $\x \in \R^n$, $\delta \x \in V_{r(t)+1}$ and $\x' := \x + \delta \x$. \\
    
    Since $\delta \x \in V_{r(t)+1}$, then we can write it in coordinate with respect to the base $\{ v_{r(t)+1}, \dots, v_n \}$ of $V_{r(t)+1}$ as 
    \begin{align*}
        \delta \x = \sum_{i=r(t)+1}^n a_i v_i
    \end{align*}
    Since the $V$ matrix of the SVD decomposition of $A$ is an orthogonal matrix, its columns $\{ v_1, \dots, v_n \}$ forms an orthonormal base of $\R^n$. Thus
    \begin{align*}
        ||\x - \x'|| = ||\delta \x|| = \sqrt{\sum_{i=r(t)+1}^n a_i^2}
    \end{align*}
    and
    \begin{align*}
        || A(\x' - \x) || = ||A \delta \x|| = ||U \Sigma V^T \delta \x||  
    \end{align*}
    but
    \begin{align*}
        U\Sigma V^T \delta \x = \sum_{i=1}^n \sigma_i (v_i^T\delta \x) u_i = \sum_{i=1}^n \sigma_i (v_i^T\sum_{j=r(t)+1}^n a_j v_j) u_i = \sum_{i=r(t)+1}^n \sigma_i a_i u_i
    \end{align*}
    which implies that 
    \begin{align*}
        || A(\x - \x') || = \sqrt{\sum_{i=r(t)+1}^n \sigma_i^2 a_i^2} \leq \sqrt{\sum_{i=r(t)+1}^n t^2 a_i^2} = t \sqrt{\sum_{i=r(t)+1}^n a_i^2} = t ||\delta \x||
    \end{align*}
    As a consequence, if we choose $||\delta \x ||$ to be $|| \delta \x || = \frac{\eta}{t}$ we have that:
    \begin{align*}
        & ||A(\x - \x')|| < \eta \\
        & ||\x - \x'|| = ||\delta \x|| = \frac{\eta}{t}
    \end{align*}
\end{proof} 

In particular, given a reconstruction algorithm $\Psi$ with accuracy $\eta>0$, we can find $\x, \x' \in \R^n$ such that $|| A(\x - \x') || < \eta$ and $||\x - \x'|| = \frac{\eta}{t}$ where $t$ is a positive number such that $r(t)<n$. As a consequence, if $A$ is ill-conditioned, we can choose $t \ll \frac{1}{2}$ such that $|| \x - \x' || \gg 2\eta$ and, by Theorem \ref{thm:estimates_of_lip},

\begin{align}
    L^\epsilon(\Psi, \tilde{y}) \geq \frac{1}{\epsilon} \Bigl(||\x - \x'|| - 2\eta \Bigr) = \frac{1}{\epsilon} \Bigl(\frac{\eta}{t} - 2\eta \Bigr) = \frac{1}{\epsilon} \Bigl(\frac{\eta - 2t\eta'}{t} \Bigr)
\end{align}

which grows linearly with $\frac{1}{t}$. In particular, the more $A$ is ill-conditioned, the more we can find a small value of $t$ such that $r(t)<n$, the most $L^\epsilon(\Psi, \tilde{y})$ is big. \\

Moreover, the proof of Theorem \ref{thm:ill_cond_implies_existence} shows that if we choose $t$ to be big, then $n - r(t)$ is big and there are a lot of couples $\x, \x'$ such that $|| \x - \x' || = \frac{\eta}{t}$ but $||A(\x-\x') ||<\eta$, but since $t$ is big, $\x$ and $\x'$ are not very far from each other. Conversely, if we reduce $t$, then the number of couples $\x, \x'$ reduces, but their required distance grows. Thus, there is a trade-off between the number of unstable couples $\x, \x'$ and their distance.

\subsection{Tikhonov-Regularized Inverse Problems}
Classically, when $A \in \R^{n \times n}$ is ill-conditioned, then Problem \eqref{eq:disc_fred_eq} is solved by solving the regularized formulation

\begin{align}\label{eq:reg_inverse_problem}
    \x_\lambda = \arg\min_{\x \in \R^n} \frac{1}{2} || A\x - y||^2 + \frac{\lambda}{2} ||L\x ||^2
\end{align}

where the first term enforces the solution $\x^*$ to fit the data well, while the second term is the Tikhonov functional, with $\lambda>0$ regularization parameter, $L \in \R^{n \times n}$ well-conditioned matrix (usually, identity or forward-difference operator). It is known that the solution of \eqref{eq:reg_inverse_problem} is way more stable then the direct solution of \eqref{eq:disc_fred_eq}. This can be related to the analysis above by observing that \eqref{eq:reg_inverse_problem} can be rewritten as

\begin{align}\label{eq:tik_extended_formulation}
    \x_\lambda = \arg\min_{\x \in \R^n} \frac{1}{2} || A^{(\lambda;L)} \x - \tilde{y} ||^2
\end{align}

where $A^{(\lambda;L)} \in \R^{2n \times n}$ and $\tilde{y} \in \R^{2n}$ are the extended matrix and the extended data, respectively, defined as

\begin{align}\label{eq:extended_definition}
\setlength\arraycolsep{2pt}
A^{(\lambda;L)} = \left[\begin{array}{c}
A \\
\hline
\lambda L
\end{array}\right] \in \R^{2n \times n} \quad \tilde{y} = \left[\begin{array}{c}
y \\
\hline
0
\end{array}\right] \in \R^{2n}
\end{align}

thus, the solution $\x_\lambda$ of \eqref{eq:reg_inverse_problem}, is the solution of an extended inverse problem

\begin{align}
    \tilde{y} = A^{(\lambda; L)}\x
\end{align}

It is known in literature, that the results of adding a Tikhonov regularation scheme to the solution of an inverse problem, lead to a better conditioned problem, where the matrix $A^{(\lambda; L)}$ is, under assumptions on $\lambda$, well-conditioned. \\

Suppose we now apply a reconstruction algorithm $\Psi$ to the extended inverse problem, with accuracy $\eta>0$, i.e. $\Psi(A^{(\lambda; L)}x) \approx_\eta x$ $\forall x \in \R^n$. We want to show that this reconstruction is stable. To do that, we prove the reverse of Theorem \ref{thm:ill_cond_implies_existence}.

\begin{theorem}
    Let $\eta>0$ and $x, x' \in \R^n$ such that $||A(x-x')||<\eta$. Then, it is possible to choose $x, x' \in \R^n$ s.t. $|| x - x' ||\gg2\eta$ if and only if $A$ is ill-conditioned.
\end{theorem}

\begin{proof}
    $(\leftarrow)$ is a consequence of Theorem \ref{thm:ill_cond_implies_existence}.
    
    $(\rightarrow)$ By contraddiction, assume $A$ is ill-conditioned. We want to prove that $|| A(x-x')||<\eta$ implies $|| x - x' ||<\eta$. \\ 
    
    Since $A$ is well-conditioned, its lower singular value $\sigma_n$ is sufficiently high. We assume $\sigma_n > 1$ to simplify the proof. Let $\delta x := x-x'$. Then, by hypothesis, $|| A\delta x || < \eta$. Since $\delta x \in \R^n$, we can write it in coordinates with respect to the (orthonormal) basis of $\R^n$ defined by the columns of the matrix $V$, where $A = U \Sigma V^T$ is the SVD decomposition of $A$, as
    
    \begin{align*}
        \delta x = \sum_{i=1}^n a_i v_i
    \end{align*}
    
    thus
    
    \begin{align*}
        A\delta x = U\Sigma V^T \delta x = \sum_{i=1}^n a_i U \Sigma V^T v_i = \sum_{i=1}^n a_i \sigma_i u_i
    \end{align*}
    
    which implies that
    
    \begin{align*}
        \eta^2 > ||A\delta x||^2 = \sum_{i=1}^n a_i^2 \sigma_i^2 \geq n \sum_{i=1}^n a_i^2 = n||\delta x ||^2 > || \delta x ||^2
    \end{align*}
    
    and
    
    \begin{align*}
        || \delta x || < \eta
    \end{align*}
    
    which is a contraddiction.
\end{proof}

As a consequence, if $\lambda>0$ is chosen such that $A^{(\lambda; L)}$ is sufficiently well-conditioned, we can prove that there are not $x, x' \in \R^n$ that generate instability as a consequence of Theorem \ref{thm:estimates_of_lip}.


\subsection{Conclusion of the section}
To conclude this section, we briefly summarize the results we obtained. We began by an ill-conditioned inverse problem $y = Ax$ where the goal is to recover $x$ given $y$. The ill-conditioning of this problem implies that we can define very small values of $t>0$ such that $r(t) < n$ for $A$. \\

Given a very accurate continuous reconstruction algorithm $\Psi:\R^n \to \R^n$ with accuracy $\eta>0$, the ill-conditioning of the inverse problem implied that we can find some points $x, x' \in \R^n$ such that $||x-x'||\gg 2\eta$ while $||A(x -x') || < \eta$. The existence of those points, implies that to achieve accuracy $\eta>0$, our reconstruction algorithm $\Psi$ must have a huge local Lipschitz constant, which can be lower-bounded by a quantity that depends on the lowest singular value of $A$. Having a large local Lipschitz constant, means that the $\Phi$ must be very unstable to small perturbation of the input, which can be written as being $\delta$-stable only for very large values of $\delta$. This observation conclude the introduction. The next step is to show that a very accurate reconstruction algorithm $\Psi$ exists, which will implies instability, and to investigate how one can solve this problem (RISING).
